From Classical To Quantum Gravity: Introduction to Loop Quantum Gravity

We present an introduction to the canonical quantization of gravity performed in loop quantum gravity, based on lectures held at the 3rd quantum geometry and quantum gravity school in Zakopane in 2011. A special feature of this introduction is the inclusion of new proposals for coupling matter to gravity that can be used to deparametrize the theory, thus making its dynamics more tractable. The classical and quantum aspects of these new proposals are explained alongside the standard quantization of vacuum general relativity in loop quantum gravity.

==> SolvConstraints.tex <==
We are looking for solutions to the constraints in the quantum theory, hence we want to find states that are annihilated by the constraint operators, that is '$\hat{C}\psi_{\rm phys}=0$'. In general the constraint operators $\hat{C}$ are complicated functions of holonomies and fluxes and we are looking for the value zero in their spectra. 
In the simplest case the operators that we need to consider are bounded and their spectra is disrete. Then the operators are defined on the whole Hilbert space $\Hkin$ and the eigenvectors of the operators are elements of $\Hkin$. As we will see later on this is the case for the Gau\ss{} constraint operator. However, often the physically interesting operators are unbounded and in this case they are only defined on a dense subset of $\Hkin$. Futhermore, in general, the spectrum of the operators will have a continuous part and the associated (generalized) eigenvectors will no longer belong to $\Hkin$. In our case this situation occurs whenever 
zero will not  lie in the discrete part of the spectrum of the constraint operators. A similar situation occurs already in standard quantum mechanics for the momentum  and position operators both being unbounded. The spectrum of the momentum operator $\hat{p}=-i\hbar \frac{d}{dx}$ is the real line and the (generalized) eigenfunctions are plane waves $\psi_k(x)=e^{ikx}$ that are not square integrable on $(\mathbb{R},dx)$ and thus no element of ${\cal H}_{QM}=L_2(\mathbb{R},dx)$. Likewise, the generalized eigenfunctions of the position operator are delta functions and therefore also no elements of ${\cal H}_{QM}$.
In those cases one has to look for solutions in a larger space than ${\cal H}_{QM}$ and, in the case of LQG,  ${\cal H}_{\rm kin}$ respectively. The mathematical framework that can be used here are so called rigged Hilbert spaces (also called Gelfand triples). They consists of a sequence of spaces
\be
 {\cal D}\subset {\cal H}\subset {\cal D}^\times
 \ee
where ${\cal D}$ is a dense subspace of $\cal H$ endowed with its own intrinsic topology, that is assumed to be stronger than the one induced from $\cal H$ and ${\cal D}^\times$ is the dual space of $\cal D$ containing all continuous anti-linear functionals on $\cal D$. The dense subspace is usually chosen by the requirement that it is the largest dense subspace of $\cal H$ such that it is an invariant domain for arbitrary powers of the elementary operators. For instance in the case of quantum mechanics the dense subset is the ${\cal S}(\mathbb{R})$, the Schwartz space of smooth rapidly decreasing functions on $\mathbb{R}$. Associated with a given Gelfand triple
 there always exist a second rigged Hilbert space
\be
\label{Gelfand2}
 {\cal D}\subset {\cal H}\subset {\cal D}^\prime
 \ee
 which consists of $\cal D,\cal H$ and the dual space ${\cal D}^\prime$ of all linear and continuous functionals on $\cal D$ and it is the second rigged Hilbert space that we will discuss for LQG. In the case of quantum mechanics when the spectrum has a continuous part the associated (generalized) eigenvectors expressed as Dirac ket vectors live in $\cal {D}^\times$, whereas the home of the corresponding Dirac bra vectors is the space $\cal {D}^\prime$. For LQG we restrict our discussion to the latter Gelfand' triplet in (\ref{Gelfand2}).
Let us denote with $\Dkin$ the dense subspace of $\Hkin$ and as we saw before elements of $\Dkin$ are cylindrical functions.  Apart from the dense subspace $\Dkin$ itself the rigged Hilbert space requires that $\Dkin$ is endowed with an intrinsic topology stronger than the one induced from $\Hkin$ and as far as physics is concerned it does not yield a particular choice of a topology here. In order to avoid such a choice at this stage in LQG we do not consider the topological dual space $\Dkin^\prime$ but the algebraic dual instead denoted by $\Dkin^*$. Then we look for solutions in the algebraic dual ${\cal D}_{\rm kin}^*$ that is the space of all linear but not necessarily continuous functionals $\ell$ on ${\cal D}_{\rm kin}$. ${\cal D}_{\rm kin}^*$ is naturally equipped with the weak *-topology of pointwise convergence of nets\footnote{A net, that is a generalization of a sequence,  $(\ell^\alpha)$ converges in ${\cal D}_{\rm kin}^*$ if $(\ell_\alpha(f))$ converges to $\ell(f)$ for any $f$ in ${\cal D}_{\rm kin}$.}. As before we have the following topological inclusion 
\be
{\cal D}_{\rm kin}\subset{\cal H}_{\rm kin}\subset{\cal D}_{\rm kin}^*
\ee
since any functional that converges strongly in the norm of ${\cal H}_{\rm kin}$ will also converge pointwise. 
In order to formulate a requirement for solutions to the constraints in ${\cal D}_{\rm kin}^*$ we need to extend the action of the operators from ${\cal H}_{\rm kin}$ onto ${\cal D}_{\rm kin}^*$.
On those linear functionals $\ell$ that lie in ${\cal H}_{\rm kin}$ we want the action of the dual operator to agree with the usual one on ${\cal H}_{\rm kin}$. Let us denote the extension of an operator $\hat{O}$ by $\hat{O}^\prime$ then we define
\be
\label{DefOprime}
\left[\hat{O}^\prime\ell\right](f):=\ell(\hat{O}^\dagger f)
\ee
where $\dagger$ denotes the adjoint in $\Hkin$. Now suppose we have an $\ell\in\Hkin\subset\Dkin^*$ then using Riesz representation theorem we find a unique $f_\ell\in\Hkin$ such that $\ell$ can be expressed as $\ell=\langle f_\ell, .\rangle_{\Hkin}$ where $\langle .,.\rangle_{\Hkin}$ denotes the inner product on $\Hkin$. Then we obtain
\be
\label{lSol}
\left[\hat{O}^\prime\ell\right](f)=\ell(\hat{O}^\dagger f)=\langle f_\ell, \hat{O}^\dagger f\rangle_{\Hkin}=\langle \hat{O} f_\ell,  f\rangle_{\Hkin},
\ee
which explains the use of the adjoint in equation (\ref{DefOprime}). Looking for solutions in $\Dkin^*$ corresponds to finding linear functionals that  satisfy the following requirement
\be
\left[\hat{C}^\prime\ell\right](f)=\ell(\hat{C}^\dagger f)=0\quad{\rm for\,\, all}\,\, \hat{C},f\in\Dkin
\ee
Let us denote the set of solutions to the constraints by $\Dphys^*$. In general physical operators, those that commute with all constraint operators, will be unbounded and therefore only be defined on a dense subset of the physical Hilbert space $\Hphys$ denoted by $\Dphys$, which is an invariant domain for the algebra of physical operators. The set $\Dphys^*$ is then the algebraic dual of $\Dphys$ and as before again one has also at the physical level a topological inclusion
\be
\Dphys\subset\Hphys\subset\Dphys^*
\ee
Given this situation there exists a systematic way to construct an inner product of the physical Hilbert space $\Hphys$ be means of a so called rigging map $\eta$ 
\be
\eta :\Dkin\to\Dphys^*,\quad f\mapsto \eta(f)
\ee
that maps elements in $\Dkin$ into $\Dphys^*$. $\eta(f)$ being an element of $\Dphys^*$ is a linear functional on $\Dkin$ that additionally satisfies the condition in equation (\ref{lSol}), hence 
 $[\eta(f)](\tilde{f})$ is a complex number and if in addition 
 \bea
 (i) &  \overline{[\eta(f)](\tilde{f})}=[\eta(\tilde{f})](f)\\
 (ii) & [\eta(f)](f)\geq0\quad{\rm for\,\, all}\, f,\quad [\eta(f)](f)=0 \Rightarrow f=0 \\
 (iii) & [\eta(f)](\alpha g + \beta h)= \alpha[\eta(f)](g) + \beta[\eta(f)](h) 
 \eea
 are satisfied we can use $[\eta(f)](\tilde{f})$ do define a physical inner product. The bar in (i) denotes complex conjugation. Condition (ii) is trivially satisfied since $[\eta(f)]$ is a linear functional and from (iii) we see that we cannot have $\Dphys=\Dkin$ whenever $\eta$ has a non-trivial kernel. Whether $(i,iii)$ are satisfied and thus $[\eta(.)](.)$ defines a positive semi definite sesquilinear form needs to be checked  once the explicit form of $\eta$ has been constructed. Apart from the minimal requirements (i-iii) we want the inner product to satisfy the property that adjoints with respect to the physical inner product $\langle .,.\rangle_{\rm phys}$ represent the adjoints in the corresponding kinematical case. That means that we can either first extend the operators to $\Dphys^*$ and then construct the adjoint or take the adjoint first in $\Dkin$ and then extend the adjoint operator to $\Dphys^*$ and we will obtain the same result. This yields the following condition for the physical inner product
 \be
 \label{AdjoinCond}
 \langle (\hat{O}^\prime)^\dagger\psi,\tilde{\psi}\rangle_{\rm phys} = \langle (\hat{O}^\dagger)^\prime\psi,\tilde{\psi}\rangle_{\rm phys}
 \ee
 Here we denoted the adjoint with respect to the physical inner product with the same symbol $\dagger$ we used in the kinematical case. Furthermore, the rigging map needs to be constructed in such a way that the physical operators $\hat{O}$ defined on $\Hphys$ or $\Dphys$ respectively preserve the space of solutions $\Dphys^*$, that means
 \be
 \hat{O}^\prime\eta(f)=\eta(\hat{O}f)\quad{\rm for\,\, all}\,\, f\in{\Dkin}
 \ee
 A physical inner product can then be defined  as
 \be
 \label{physInn}
 \langle\psi,\tilde{\psi}\rangle_{\rm phys} = \langle\eta(f),\eta(\tilde{f})\rangle_{\rm phys}:=[\eta(\tilde{f})](f)
 \ee
 With that definition of an inner product the condition in (\ref{AdjoinCond}) is automatically satisfied
 \bea
  \langle (\hat{O}^\prime)^\dagger\psi,\tilde{\psi}\rangle_{\rm phys} &=& \langle \psi,\hat{O}^\prime\tilde{\psi}\rangle_{\rm phys}\nn  \\
  &=&\langle\eta(f),\eta(\hat{O}\tilde{f})\rangle_{\rm phys}\nn \\
  &=&[\eta(\hat{O}\tilde{f})](f)=[\hat{O}^\prime\eta(\tilde{f})](f)=[\eta(\tilde{f})](\hat{O}^\dagger f)\nn \\
  &=&\langle\eta(\hat{O}^\dagger f),\eta(\tilde{f})\rangle_{\rm phys}\nn \\
  &=& \langle (\hat{O}^\dagger)^\prime\psi,\tilde{\psi}\rangle_{\rm phys}
  \eea
  An example how a rigging map can be explicitly constructed is the so called group averaging procedure. Consider a set of constraint operators ${\hat{C}_I}$ where $I$ labels the individual constraints that are self-adjoint and their first class algebra is a Lie algebra, then we can define unitary operators by using the exponential map
  \be
  \hat{U}(g)=\exp\left(i\sum\limits_I \alpha^I\hat{C}_I\right)
  \ee
  with paramters $t\in T\subset\R$ yielding a unitary representation of the Lie group. The condition that a function $f$ is annihilated by the infinitesimal generators of the constraints carries over to the requirement that 
  a linear functional that is a solution of the constraints if it is invariant under the action of those unitary operators, that is for $f\in\Dkin$
  \be
  [(\hat{U}(t))^\prime](f)=\ell((\hat{U}(t))^\dagger f) = \ell(f)\quad{\rm for\,\, all}\,\, t\in T
  \ee
Using the unitary operators we can define a projector on physical states given by
\be
\label{Proj}
\hat{P}=\int\limits_G d\mu_H(g)\hat{U}(g)
\ee
where $\mu_H$ denotes Haar measure on $G$. The properties of the Haar measure that it is invariant under right and left translation are important for showing that the projector defined above indeed projects on physical states as can be seen below
\bea
\hat{U}(g)\hat{P}f&=&
\hat{U}(g)\int\limits_G d\mu_H(h)\hat{U}(h)f\nn \\
&=&\int\limits_G d\mu_H(h)\hat{U}(g)\hat{U}(h)f\nn \\
&=&\int\limits_G d\mu_H(h)\hat{U}(gh)f\nn \\
&=&\int\limits_G d\mu_H(g^{-1}\tilde{g})\hat{U}(\tilde{g})f\nn \\
&=&\hat{P}f
\eea
In the third line we used that $G$ is a group, in the fourth line we introduced the new integration variable $\tilde{g}:=gh$ and in the one before the last line we used that $\mu_h$ is invariant under translations. The rigging map $\eta$ can now be expressed in term of the projector defined in  (\ref{Proj})
\be
\eta : \Dkin \to \Hphys \subset \Dphys^*\quad f\mapsto \eta(f):=\int\limits_G d\mu(g)_H\langle \hat{U}^(g)f,.\rangle_{\rm kin}
\ee
and the physical inner product can then be defined as
\be
\langle\eta(f),\eta(\tilde{f})\rangle_{\rm phys}:=[\eta(\tilde{f})](f)
\ee
Likewise to the case of quantum mechanics where the Dirac bra and ket vectors in the spaces ${\cal D}^\times$ and ${\cal D}^\prime$  are distributions on $\cal D$ also here the linear functional $\eta(f)$ defined above is a distribution on $\Dkin$. In this sense the rigged Hilbert space framework combines Hilbert spaces with distribution theory and allows us to understand the case of unbounded operators with continuous spectra along the lines of the standard language used in quantum theory. 




